Differential Equation Based Path Integral for System-Bath Dynamics

We propose the differential equation based path integral (DEBPI) method to simulate the real-time evolution of open quantum systems. In this method, a system of partial differential equations is derived based on the continuation of a classical numerical method called iterative quasi-adiabatic propagator path integral (i-QuAPI). While the resulting system has infinite equations, we introduce a reasonable closure to obtain a series of finite systems. New numerical schemes can be derived by discretizing these differential equations. It is numerically verified that in certain cases, by selecting appropriate systems and applying suitable numerical schemes, the memory cost required in the i-QuAPI method can be significantly reduced.

==> sections/extraNotes.tex <==
\ki{Remove this section after integrating the contents to other sections.}

For $h$ given by \eqref{contPath},
 the initial value $A(0,h)$ can be given by
\begin{equation}
    \begin{split}
        A(0,h) =& \mel{r_0^+}{\rho_s(0)}{r_0^-}  
        \e^{-\ii\left(\mel{r_0^+}{H_0}{r_0^+}-\mel{r_0^-}{H_0}{r_0^-}\right)\tau_1} \\
        & \prod_{j=1}^{D-1}
        \Bigg(
        \e^{-\ii\big(\mel{r_j^+}{H_0}{r_j^+}-\mel{r_j^-}{H_0}{r_j^-}\big)\tau_{j+1}}
        \left(-\ii\mel{r_j^+}{H_0}{r_{j-1}^+}\delta_{\sgn_j}^+ + \ii \mel{r_{j-1}^-}{H_0}{r_j^-}\delta_{\sgn_j}^-\right)
        \Bigg) \\
        &\e^{-\ii\big(\mel{r_D^+}{H_0}{r_D^+}-\mel{r_D^-}{H_0}{r_D^-}\big) \left(T-\sum_{j=1}^D \tau_j\right) }
        \left(-\ii\mel{r_D^+}{H_0}{r_{D-1}^+}\delta_{\sgn_D}^+ + \ii \mel{r_{D-1}^-}{H_0}{D_j^-}\delta_{\sgn_D}^-\right)
        \\
        &\exp\left( -\int_{0}^T \dif x_1 \int_0^{x_1} \dif x_2
        (h^+(x_1)-h^-(x_1))
        (h^+(x_2)\tilde{\eta}(x_1-x_2)-h^-(x_2)\tilde{\eta}^*(x_1-x_2))
        \right)
    \end{split}
\end{equation}
where $\delta_{\sgn_j}^+=\begin{cases}
1,\text{ if } \sgn_j = + \\
0,\text{ if } \sgn_j = - \\
\end{cases}$, 
$\delta_{\sgn_j}^-=\begin{cases}
0,\text{ if } \sgn_j = + \\
1,\text{ if } \sgn_j = - \\
\end{cases}$.

% For time $[0,t)$, if the path is given by
%  $g$, which has the same form of \eqref{contPath},
%  we add $\tilde{\cdot}$ for all variables.
% \begin{equation}
%     \begin{split}
%         &\mel{\tilde{r}_0^+}{\rho_s(0)}{\tilde{r}_0^-}
%          \e^{-\ii\left(\mel{\tilde{r}_0^+}{H_0}{\tilde{r}_0^+}-\mel{\tilde{r}_0^-}{H_0}{\tilde{r}_0^-}\right)\tilde{\tau}_1} \\
%         &\prod_{j=1}^{\tilde{D}}
%         \Bigg(
%         \e^{-\ii\big(\mel{\tilde{r}_j^+}{H_0}{\tilde{r}_j^+}-\mel{\tilde{r}_j^-}{H_0}{\tilde{r}_j^-}\big)\tilde{\tau}_{j+1}}
%         \left(-\ii\mel{\tilde{r}_j^+}{H_0}{\tilde{r}_{j-1}^+}\delta_{\widetilde{\sgn}_j}^+ + \ii \mel{\tilde{r}_{j-1}^-}{H_0}{\tilde{r}_j^-}\delta_{\widetilde{\sgn}_j}^-\right)
%         \Bigg) \\
%         &\delta_{\tilde{r}_{\tilde{D}}^+}^{r_0^+}
%         \delta_{\tilde{r}_{\tilde{D}}^-}^{r_0^-}
%         \e^{-\ii\left(\mel{{r}_0^+}{H_0}{{r}_0^+}-\mel{{r}_0^-}{H_0}{{r}_0^-}\right){\tau}_1}
%         \\
%         &\prod_{j=1}^D
%         \Bigg(
%         \e^{-\ii\big(\mel{r_j^+}{H_0}{r_j^+}-\mel{r_j^-}{H_0}{r_j^-}\big)\tau_{j+1}}
%         \left(-\ii\mel{r_j^+}{H_0}{r_{j-1}^+}\delta_{\sgn_j}^+ + \ii \mel{r_{j-1}^-}{H_0}{r_j^-}\delta_{\sgn_j}^-\right)
%         \Bigg) \\
%         &\exp\Bigg(
%         -\int_0^t\dif x_1 \int_{\max\{0,x_1-T\}}^{x_1}\dif x_2
%         (g^+(x_1)-g^-(x_1))
%         (g^+(x_2)\tilde{\eta}(x_1-x_2)-g^-(x_2)\tilde{\eta}^*(x_1-x_2)) \\
%         &\quad -\int_t^{t+T}
%         \dif x_1 \int_{\max\{0,x_1-T\}}^{x_1}\dif x_2
%         (h^+(x_1-t)-h^-(x_1-t))
%         (g^+(x_2)\tilde{\eta}(x_1-x_2)-g^-(x_2)\tilde{\eta}^*(x_1-x_2)) \\
%         &\quad -\int_{0}^T \dif x_1 \int_0^{x_1} \dif x_2
%         (h^+(x_1)-h^-(x_1))
%         (h^+(x_2)\tilde{\eta}(x_1-x_2)-h^-(x_2)\tilde{\eta}^*(x_1-x_2))
%         \Bigg)
%     \end{split}
% \end{equation}
% Therefore,
% \begin{equation}
%     \begin{split}
%     A(t,h) =&\sum_{\tilde{D}=0}^\infty
%         \sum_{(\tilde{r}_0^+,\tilde{r}_0^-)\in\mathcal{S}^2}
%         \sum_{ \widetilde{\sgn} \in \{+,-\}^{\tilde{D}} }
%         \int_{0}^t \dif \tilde{\tau}_1
%         \int_{0}^{t-\tilde{\tau}_1} \dif \tilde{\tau}_2
%         \cdots 
%         \int_{0}^{t-\tilde{\tau}_1-\cdots-\tilde{\tau}_{\tilde{D}-1}} \dif \tilde{\tau}_{\tilde{D}}
%         \\
%         &\mel{\tilde{r}_0^+}{\rho_s(0)}{\tilde{r}_0^-}
%          \e^{-\ii\left(\mel{\tilde{r}_0^+}{H_0}{\tilde{r}_0^+}-\mel{\tilde{r}_0^-}{H_0}{\tilde{r}_0^-}\right)\tilde{\tau}_1} \\
%         &\prod_{j=1}^{\tilde{D}}
%         \Bigg(
%         \e^{-\ii\big(\mel{\tilde{r}_j^+}{H_0}{\tilde{r}_j^+}-\mel{\tilde{r}_j^-}{H_0}{\tilde{r}_j^-}\big)\tilde{\tau}_{j+1}}
%         \left(-\ii\mel{\tilde{r}_j^+}{H_0}{\tilde{r}_{j-1}^+}\delta_{\widetilde{\sgn}_j}^+ + \ii \mel{\tilde{r}_{j-1}^-}{H_0}{\tilde{r}_j^-}\delta_{\widetilde{\sgn}_j}^-\right)
%         \Bigg) \\
%         &\delta_{\tilde{r}_{\tilde{D}}^+}^{r_0^+}
%         \delta_{\tilde{r}_{\tilde{D}}^-}^{r_0^-}
%         \e^{-\ii\left(\mel{{r}_0^+}{H_0}{{r}_0^+}-\mel{{r}_0^-}{H_0}{{r}_0^-}\right){\tau}_1}
%         \\
%         &\prod_{j=1}^D
%         \Bigg(
%         \e^{-\ii\big(\mel{r_j^+}{H_0}{r_j^+}-\mel{r_j^-}{H_0}{r_j^-}\big)\tau_{j+1}}
%         \left(-\ii\mel{r_j^+}{H_0}{r_{j-1}^+}\delta_{\sgn_j}^+ + \ii \mel{r_{j-1}^-}{H_0}{r_j^-}\delta_{\sgn_j}^-\right)
%         \Bigg) \\
%         &\exp\Bigg(
%         -\int_0^t\dif x_1 \int_{\max\{0,x_1-T\}}^{x_1}\dif x_2
%         (g^+(x_1)-g^-(x_1))
%         (g^+(x_2)\tilde{\eta}(x_1-x_2)-g^-(x_2)\tilde{\eta}^*(x_1-x_2)) \\
%         &\quad -\int_t^{t+T}
%         \dif x_1 \int_{\max\{0,x_1-T\}}^{x_1}\dif x_2
%         (h^+(x_1-t)-h^-(x_1-t))
%         (g^+(x_2)\tilde{\eta}(x_1-x_2)-g^-(x_2)\tilde{\eta}^*(x_1-x_2)) \\
%         &\quad -\int_{0}^T \dif x_1 \int_0^{x_1} \dif x_2
%         (h^+(x_1)-h^-(x_1))
%         (h^+(x_2)\tilde{\eta}(x_1-x_2)-h^-(x_2)\tilde{\eta}^*(x_1-x_2))
%         \Bigg)
%     \end{split}
% \end{equation}

For simplicity,
 we write $A(t,h)$ as

where

Therefore, according to \eqref{Asimplified} 
\begin{equation}
\begin{split}
    \frac{\partial}{\partial \tau_1}A(t,h)
    =& \sum_{\tilde{D}=0}^\infty \sum_{(\tilde{r}_0^+,\tilde{r}_0^-)\in\mathcal{S}^2}
    \sum_{\widetilde{\sgn}\in\{+,-\}^{\tilde{D}}}
    \int_0^t \dif \tilde{\tau}_{\tilde{D}}
    \int_0^{\tilde{\tau}_{\tilde{D}}} \dif \tilde{\tau}_{\tilde{D}-1}\cdots
    \int_{0}^{\tilde{\tau}_2} \dif \tilde{\tau}_1
    X(g)
    \delta_{\tilde{r}_{\tilde{D}}^+}^{r_0^+}
    \delta_{\tilde{r}_{\tilde{D}}^-}^{r_0^-}
    \frac{\partial}{\partial \tau_1} Y(h)
    \e^{Z(g,h)} \\
    &+ \sum_{\tilde{D}=0}^\infty \sum_{(\tilde{r}_0^+,\tilde{r}_0^-)\in\mathcal{S}^2}
    \sum_{\widetilde{\sgn}\in\{+,-\}^{\tilde{D}}}
    \int_0^t \dif \tilde{\tau}_{\tilde{D}}
    \int_0^{\tilde{\tau}_{\tilde{D}}} \dif \tilde{\tau}_{\tilde{D}-1}\cdots
    \int_{0}^{\tilde{\tau}_2} \dif \tilde{\tau}_1
    X(g)
    \delta_{\tilde{r}_{\tilde{D}}^+}^{r_0^+}
    \delta_{\tilde{r}_{\tilde{D}}^-}^{r_0^-}
    Y(h)
    \frac{\partial}{\partial \tau_1} Z(g,h) \e^{Z(g,h)}
\end{split}
\end{equation}
% \begin{equation}
%     \begin{split}
%         \frac{\partial}{\partial t}A(t,h)
%         =& \frac{\partial}{\partial t}\left(\sum_{(\tilde{r}_0^+,\tilde{r}_0^-)\in\mathcal{S}^2}
%         \mel{\tilde{r}_0^+}{\rho_s(0)}{\tilde{r}_0^-}
%         \e^{-\ii\left(\mel{\tilde{r}_0^+}{H_0}{\tilde{r}_0^+}-\mel{\tilde{r}_0^-}{H_0}{\tilde{r}_0^-}\right) t}
%         \delta_{\tilde{r}_{\tilde{D}}^+}^{r_0^+}
%         \delta_{\tilde{r}_{\tilde{D}}^-}^{r_0^-}
%         Y(h)
%         \e^{Z(g,h)}\right)\\
%         &+ \frac{\partial}{\partial t}\left(
%         \sum_{\tilde{D}=1}^\infty
%         \sum_{(\tilde{r}_0^+,\tilde{r}_0^-)\in\mathcal{S}^2}
%         \sum_{ \widetilde{\sgn} \in \{+,-\}^{\tilde{D}} }
%         \int_0^t \dif\tilde{\tau}_{\tilde{D}}
%         \int_0^{\tilde{\tau}_{\tilde{D}}} \dif \tilde{\tau}_{{\tilde{D}}-1}
%         \cdots
%         \int_0^{\tilde{\tau}_2} \dif \tilde{\tau}_1
%         X(g)
%         \delta_{\tilde{r}_{\tilde{D}}^+}^{r_0^+}
%         \delta_{\tilde{r}_{\tilde{D}}^-}^{r_0^-}
%         Y(h)
%         \e^{Z(g,h)}\right) \\
%         =& \sum_{(\tilde{r}_0^+,\tilde{r}_0^-)\in\mathcal{S}^2}
%         \frac{\partial}{\partial t}\left(\mel{\tilde{r}_0^+}{\rho_s(0)}{\tilde{r}_0^-}
%         \e^{-\ii\left(\mel{\tilde{r}_0^+}{H_0}{\tilde{r}_0^+}-\mel{\tilde{r}_0^-}{H_0}{\tilde{r}_0^-}\right) t}\delta_{\tilde{r}_{\tilde{D}}^+}^{r_0^+}
%         \delta_{\tilde{r}_{\tilde{D}}^-}^{r_0^-}
%         Y(h)
%         \e^{Z(g,h)}\Big\vert_{\tilde{D}=0}\right)\\
%         &+ 
%         \sum_{\tilde{D}=1}^\infty
%         \sum_{(\tilde{r}_0^+,\tilde{r}_0^-)\in\mathcal{S}^2}
%         \sum_{ \widetilde{\sgn} \in \{+,-\}^{\tilde{D}} }
%         \int_0^{\tilde{\tau}_{t}} \dif \tilde{\tau}_{{\tilde{D}}-1}
%         \cdots
%         \int_0^{\tilde{\tau}_2} \dif \tilde{\tau}_1
%         X(g)\Big\vert_{\tilde{\tau}_{\tilde{D}}=t}
%         \delta_{\tilde{r}_{\tilde{D}}^+}^{r_0^+}
%         \delta_{\tilde{r}_{\tilde{D}}^-}^{r_0^-}
%         Y(h)
%         \e^{Z(g,h)}\Big\vert_{\tilde{\tau}_{\tilde{D}}=t} \\
%         &+ \sum_{\tilde{D}=1}^\infty
%         \sum_{(\tilde{r}_0^+,\tilde{r}_0^-)\in\mathcal{S}^2}
%         \sum_{ \widetilde{\sgn} \in \{+,-\}^{\tilde{D}} }
%         \int_0^t \dif\tilde{\tau}_{\tilde{D}}
%         \int_0^{\tilde{\tau}_{\tilde{D}}} \dif \tilde{\tau}_{{\tilde{D}}-1}
%         \cdots
%         \int_0^{\tilde{\tau}_2} \dif \tilde{\tau}_1
%         \frac{\partial}{\partial t}\left(X(g)
%         \delta_{\tilde{r}_{\tilde{D}}^+}^{r_0^+}
%         \delta_{\tilde{r}_{\tilde{D}}^-}^{r_0^-}
%         Y(h)
%         \e^{Z(g,h)}\right)
%     \end{split}
% \end{equation}

\begin{equation}
    \begin{split}
        \frac{\partial}{\partial t}A(t,h)
        =& \sum_{\tilde{D}=1}^\infty
        \sum_{(\tilde{r}_0^+,\tilde{r}_0^-)\in\mathcal{S}^2}
        \sum_{ \widetilde{\sgn} \in \{+,-\}^{\tilde{D}} }
        \int_0^{\tilde{\tau}_{t}} \dif \tilde{\tau}_{{\tilde{D}}-1}
        \cdots
        \int_0^{\tilde{\tau}_2} \dif \tilde{\tau}_1
        X(g)\Big\vert_{\tilde{\tau}_{\tilde{D}}=t}
        {\color{red}{\delta_{\tilde{r}_{\tilde{D}}^+}^{r_0^+}
        \delta_{\tilde{r}_{\tilde{D}}^-}^{r_0^-} }}
        Y(h)
        \e^{Z(g,h)}\Big\vert_{\tilde{\tau}_{\tilde{D}}=t} \\
        &+ \sum_{\tilde{D}=0}^\infty
        \sum_{(\tilde{r}_0^+,\tilde{r}_0^-)\in\mathcal{S}^2}
        \sum_{ \widetilde{\sgn} \in \{+,-\}^{\tilde{D}} }
        \int_0^t \dif\tilde{\tau}_{\tilde{D}}
        \int_0^{\tilde{\tau}_{\tilde{D}}} \dif \tilde{\tau}_{{\tilde{D}}-1}
        \cdots
        \int_0^{\tilde{\tau}_2} \dif \tilde{\tau}_1
        \frac{\partial}{\partial t}X(g)
        \delta_{\tilde{r}_{\tilde{D}}^+}^{r_0^+}
        \delta_{\tilde{r}_{\tilde{D}}^-}^{r_0^-}
        Y(h)
        \e^{Z(g,h)} \\
        &+\sum_{\tilde{D}=0}^\infty
        \sum_{(\tilde{r}_0^+,\tilde{r}_0^-)\in\mathcal{S}^2}
        \sum_{ \widetilde{\sgn} \in \{+,-\}^{\tilde{D}} }
        \int_0^t \dif\tilde{\tau}_{\tilde{D}}
        \int_0^{\tilde{\tau}_{\tilde{D}}} \dif \tilde{\tau}_{{\tilde{D}}-1}
        \cdots
        \int_0^{\tilde{\tau}_2} \dif \tilde{\tau}_1
        X(g)
        \delta_{\tilde{r}_{\tilde{D}}^+}^{r_0^+}
        \delta_{\tilde{r}_{\tilde{D}}^-}^{r_0^-}
        Y(h)
        \frac{\partial}{\partial t}Z(g,h)\e^{Z(g,h)}
    \end{split}
\end{equation}

For a fixed path $g$,
\begin{equation}
    \frac{\partial}{\partial t}X(g)
        \delta_{\tilde{r}_{\tilde{D}}^+}^{r_0^+}
        \delta_{\tilde{r}_{\tilde{D}}^-}^{r_0^-}
        Y(h)
        \e^{Z(g,h)}
    = -\ii \left(\mel{\tilde{r}_{\tilde{D}}^+}{H_0}{\tilde{r}_{\tilde{D}}^+} -\mel{\tilde{r}_{\tilde{D}}^-}{H_0}{\tilde{r}_{\tilde{D}}^-}\right) X(g) \delta_{\tilde{r}_{\tilde{D}}^+}^{r_0^+}
        \delta_{\tilde{r}_{\tilde{D}}^-}^{r_0^-}
        Y(h)
        \e^{Z(g,h)}
\end{equation}
and 
\begin{equation}
\begin{split}
    &X(g)
    \delta_{\tilde{r}_{\tilde{D}}^+}^{r_0^+}
    \delta_{\tilde{r}_{\tilde{D}}^-}^{r_0^-}        \frac{\partial}{\partial \tau_1} Y(h)
    \e^{Z(g,h)} \\
    =& \Big(-\ii \big(
    \mel{r_0^+}{H_0}{r_0^+} - \mel{r_0^-}{H_0}{r_0^-}
    \big)
    + \ii
    \big(\mel{r_D^+}{H_0}{r_D^-} - \mel{r_D^-}{H_0}{r_D^-}\big)
    \Big)
    X(g) \delta_{\tilde{r}_{\tilde{D}}^+}^{r_0^+}
    \delta_{\tilde{r}_{\tilde{D}}^-}^{r_0^-}
    Y(h)
    \e^{Z(g,h)}.
\end{split}
\end{equation}
Therefore,
\begin{equation}
\begin{split}
    &\frac{\partial}{\partial t}X(g)
    \delta_{\tilde{r}_{\tilde{D}}^+}^{r_0^+}
    \delta_{\tilde{r}_{\tilde{D}}^-}^{r_0^-}
    Y(h)
    \e^{Z(g,h)}
    - X(g)
    \delta_{\tilde{r}_{\tilde{D}}^+}^{r_0^+}
    \delta_{\tilde{r}_{\tilde{D}}^-}^{r_0^-}        \frac{\partial}{\partial \tau_1} Y(h)
    \e^{Z(g,h)} \\
    =& - \ii\big(\mel{r_D^+}{H_0}{r_D^-} - \mel{r_D^-}{H_0}{r_D^-}\big)
    X(g) \delta_{\tilde{r}_{\tilde{D}}^+}^{r_0^+}
    \delta_{\tilde{r}_{\tilde{D}}^-}^{r_0^-}
    Y(h)
    \e^{Z(g,h)}.
\end{split}
\end{equation}

In addition, consider the term with $Z(g,h)$
 and $\delta_{\tilde{r}_{\tilde{D}}^+}^{r_0^+}
        \delta_{\tilde{r}_{\tilde{D}}^-}^{r_0^-}=1$,
 we have
\begin{equation}
\begin{split}
    &\frac{\partial}{\partial t}Z(g,h)
    - \frac{\partial}{\partial \tau_1}Z(g,h) \\
    =& \lim_{\dt\rightarrow 0} \frac{1}{\dt}\Bigg(
    \int_{t+T}^{t+T+\dt}\dif x_1 \int_{x_1-T}^{t+\dt} \dif x_2
    (h^+(x_1-t-\dt)-h^-(x_1-t-\dt))
    (\tilde{r}_{\tilde{D}}^+ \tilde{\eta}(x_1-x_2)
    - \tilde{r}_{\tilde{D}}^- \tilde{\eta}^*(x_1-x_2)) \\
    &\quad+
    \int_{t+T}^{t+T+\dt}\dif x_1 \int_{t+\dt}^{x_1} \dif x_2
    (h^+(x_1-t-\dt)-h^-(x_1-t-\dt)) \\
    &\qquad(h^+(x_2-t-\dt) \tilde{\eta}(x_1-x_2)
    - h^-(x_2-t-\dt) \tilde{\eta}^*(x_1-x_2))
    \Bigg) \\
    &= \int_{t}^{t+T}\dif x_2
    (h^+(T) - h^-(T))(h^+(x_2-t)\tilde{\eta}(T-x_2+t)
    -h^-(x_2-t)\tilde{\eta}^*(T-x_2+t)
\end{split}
\end{equation}

For the rest term
\begin{equation}
\begin{split}
    X(g)\Bigg\vert_{\tilde{\tau}_D=t}
    =&\mel{\tilde{r}_0^+}{\rho_s(0)}{\tilde{r}_0^-}
     \e^{-\ii\left(\mel{\tilde{r}_0^+}{H_0}{\tilde{r}_0^+}-\mel{\tilde{r}_0^-}{H_0}{\tilde{r}_0^-}\right)\tilde{\tau}_1} \\
    &\prod_{j=1}^{\tilde{D}-2}
    \Bigg(
    \e^{-\ii\big(\mel{\tilde{r}_j^+}{H_0}{\tilde{r}_j^+}-\mel{\tilde{r}_j^-}{H_0}{\tilde{r}_j^-}\big)(\tilde{\tau}_{j+1}-\tilde{\tau}_j)}
    \left(-\ii\mel{\tilde{r}_j^+}{H_0}{\tilde{r}_{j-1}^+}\delta_{\sgn_j}^+ + \ii \mel{\tilde{r}_{j-1}^-}{H_0}{\tilde{r}_j^-}\delta_{\sgn_j}^-\right)
    \Bigg) \\
    &\e^{-\ii\big(\mel{\tilde{r}_{\tilde{D}}^+}{H_0}{\tilde{r}_{\tilde{D}}^+}-\mel{\tilde{r}_{\tilde{D-1}}^-}{H_0}{\tilde{r}_{\tilde{D-1}}^-}\big)(t-\tilde{\tau}_{\tilde{D}-1})} \\
    &\left(-\ii\mel{\tilde{r}_{\tilde{D}-1}^+}{H_0}{\tilde{r}_{{\tilde{D}}-2}^+}\delta_{\sgn_{\tilde{D}-1}}^+ + \ii \mel{\tilde{r}_{{\tilde{D}}-2}^-}{H_0}{\tilde{r}_{\tilde{D}-1}^-}\delta_{\sgn_{\tilde{D}-1}}^-\right)\\
    &\left(-\ii\mel{\tilde{r}_{\tilde{D}}^+}{H_0}{\tilde{r}_{{\tilde{D}}-1}^+}\delta_{\sgn_{\tilde{D}}}^+ + \ii \mel{\tilde{r}_{{\tilde{D}}-1}^-}{H_0}{\tilde{r}_{\tilde{D}}^-}\delta_{\sgn_{\tilde{D}}}^-\right);
\end{split}
\end{equation}


==> sections/numericalScheme.tex <==
\subsection{Strang Splitting}
Strang splitting can be used in
 the numerical scheme of
 the partial differential equation \eqref{PDEoriginal}.
Consider a differential equation with the form
\begin{equation}
    \frac{\partial}{\partial t} u = L_1 u + L_2 u
\end{equation}
 with $L_1$ and $L_2$ being two operators.
The solution to the differential equation is
\begin{equation}
    u(t+\dt) = \e^{(L_1+L_2)\dt} u(t).
\end{equation}
Strang splitting suggests to approximate the solution by
\begin{equation}
    u(t+\dt) \approx \e^{L_1 \dt/2} \e^{L_2 \dt} \e^{L_1 \dt/2} u(t).
\end{equation}
With the splitting, the PDE \eqref{PDEoriginal} is separated into
 two equations.
\begin{align}
        \frac{\partial}{\partial t} A_{(s^+,s^-)}^{D,\sgn}(t,[\tau_1,\cdots,\tau_D])
        =& \frac{\partial}{\partial \tau_1} 
        A_{(s^+,s^-)}^{D,\sgn}(t,[\tau_1,\cdots,\tau_D]);
        \label{eq_advection}\\
    \begin{split}
        \frac{\partial}{\partial t} A_{(s^+,s^-)}^{D,\sgn}(t,[\tau_1,\cdots,\tau_D])
        =& -W_{(s^+,s^-)}^{D,\sgn}\left([\tau_1,\cdots,\tau_D]\right)
		A_{(s^+,s^-)}^{D,\sgn}\left(t,[\tau_1,\cdots,\tau_D]\right) \\
		&+ A_{(s^+,\hat{s}^-)}^{D+1,[-,\sgn]}
		\left(t,[0,\tau_1,\cdots,\tau_D]\right)
		+ A_{(\hat{s}^+,s^-)}^{D+1,[+,\sgn]}
		\left(t,[0,\tau_1,\cdots,\tau_D]\right).
    \end{split}
    \label{eq_source}
\end{align}
In this way, we can focus on the advection term
 and the source term respectively.

\subsection{Finite difference method}
A simple idea to solve this equation numerically
 is to apply the finite difference method.
The uniform mesh is used
 in the discretization of the simplices.

We first fix the spacial step $h_s = \frac{T}{N}$
 for $N$ is some positive integer.
For the simplex \eqref{simplex},
 the grid points are chosen to be
\begin{equation}
    \mathcal{P}_D = \left\{ \left(\frac{m_1h_s}{N},\cdots,\frac{m_Dh_s}{N}\right); m_k \in \mathbb{Z}^+, \sum_{k=1}^D m_k < N \right\},
    D = 0,\cdots,D_{\max}.
\end{equation}
Note that when $D=0$, $\mathcal{P}_0$ has one element,
 which is an empty list.

For example, if $N = 5$,
 \Cref{fig:demonstrationOfGridPoints}
 shows the grid points on the two-dimensional (triangle)
 and three-dimensional (tetrahedron) simplices.
We do not sample at the hypotenuse since
 the values on the hypotenuse are determined
 by the boundary condition
 as discussed in \Cref{boundaryCondition}.

\begin{figure}
    \centering
\begin{tikzpicture}
    \draw[->] (-0.5,0) -- (5.5,0);
    \draw[->] (0,-0.5) -- (0,5.5);
    \draw[line width = 1.5pt] (0,0) -- (5,0) -- (0,5) -- cycle;
    \filldraw[black] (5.5,0) circle node[anchor=north] {$\tau_1$};
    \filldraw[black] (0,5.5) circle node[anchor=east] {$\tau_2$};
    \filldraw[black] (5,0) circle node[anchor=north] {$T$};
    \filldraw[black] (0,5) circle node[anchor=east] {$T$};
    \filldraw[black] (0,0) circle node[anchor=north east] {$0$};
    \filldraw[red] (0,0) circle (2pt);
    \filldraw[red] (1,0) circle (2pt);
    \filldraw[red] (2,0) circle (2pt);
    \filldraw[red] (3,0) circle (2pt);
    \filldraw[red] (4,0) circle (2pt);
    \filldraw[red] (0,1) circle (2pt);
    \filldraw[red] (1,1) circle (2pt);
    \filldraw[red] (2,1) circle (2pt);
    \filldraw[red] (3,1) circle (2pt);
    \filldraw[red] (0,2) circle (2pt);
    \filldraw[red] (1,2) circle (2pt);
    \filldraw[red] (2,2) circle (2pt);
    \filldraw[red] (0,3) circle (2pt);
    \filldraw[red] (1,3) circle (2pt);
    \filldraw[red] (0,4) circle (2pt);
    
    
    \draw[->] (9,2) -- (12.5,2);
    \draw[->] (9,2) -- (9,5.5);
    \draw[->] (9,2) -- (7.3,0);
    \draw[line width = 1.5pt] (9,2) -- (12,2) -- (9,5) -- cycle;
    \draw[line width = 1.5pt] (9,2) -- (7.725,0.5) -- (12,2);
    \draw[line width = 1.5pt] (9,5) -- (7.725,0.5);
    \filldraw[black] (7.3,0) circle node[anchor=north] {$\tau_1$};
    \filldraw[black] (12.5,2) circle node[anchor=north] {$\tau_2$};
    \filldraw[black] (9,5.5) circle node[anchor=east] {$\tau_3$};
    \filldraw[black] (12,2) circle node[anchor=north] {$T$};
    \filldraw[black] (9,5) circle node[anchor=east] {$T$};
    \filldraw[black] (7.725,0.5) circle node[anchor=east] {$T$};
    
    \filldraw[red] (9,2) circle (2pt);
    \filldraw[red] (9,2.75) circle (2pt);
    \filldraw[red] (9,3.5) circle (2pt);
    \filldraw[red] (9,4.25) circle (2pt);
    \filldraw[red] (9.75,2) circle (2pt);
    \filldraw[red] (9.75,2.75) circle (2pt);
    \filldraw[red] (9.75,3.5) circle (2pt);
    \filldraw[red] (10.5,2) circle (2pt);
    \filldraw[red] (10.5,2.75) circle (2pt);
    \filldraw[red] (11.25,2) circle (2pt);

    \filldraw[blue] (9-0.31875,2-0.375) circle (2pt);
    \filldraw[blue] (9-0.31875,2.75-0.375) circle (2pt);
    \filldraw[blue] (9-0.31875,3.5-0.375) circle (2pt);
    \filldraw[blue] (9.75-0.31875,2-0.375) circle (2pt);
    \filldraw[blue] (9.75-0.31875,2.75-0.375) circle (2pt);
    \filldraw[blue] (10.5-0.31875,2-0.375) circle (2pt);
    
    \filldraw[green] (9-2*0.31875,2-2*0.375) circle (2pt);
    \filldraw[green] (9-2*0.31875,2.75-2*0.375) circle (2pt);
    \filldraw[green] (9.75-2*0.31875,2-2*0.375) circle (2pt);
    
    \filldraw[purple] (9-3*0.31875,2-3*0.375) circle (2pt);
        
\end{tikzpicture}
    \caption{The grid points on the two-dimensional simplex (red points) with $N=5$ and three dimensional simplex (points of all colors) with $N=4$.}
    \label{fig:demonstrationOfGridPoints}
\end{figure}

For a $D$-dimensional simplex with $N$ nodes on each edge,
 there are ${N+D \choose D}$ grid points in one simplex.
For different choices of initial states $(s^+,s^-)$
 and different choices of $\sgn$,
 in the spin-boson model,
 there are in total $4\times 2^D$ $D$-dimensional simplices.
Therefore, there are in total
$4\sum_{D=0}^{D_{\max}} 2^D {D+N \choose D}$
nodes in the method.

% There are two partial derivatives in \Cref{PDEoriginal},
%  we can use some finite difference scheme
%  to discretize the derivative with respect to $\tau_1$.
% For example, upwind scheme can be applied.
% Noted that for the boundary condition,
%  we apply \Cref{boundaryCondition}
%  so that we can estimate the derivative with respect to $\tau_1$.

With the grid mentioned above,
 a numerical scheme can be designed
 to evolve the whole system.
\begin{itemize}
    \item For each set of parameters
    $D = 0,\cdots,D_{\max}$, $(s^+,s^-) = (\pm1,\pm1)$
    and $p\in\mathcal{P}_D$
    compute 
    $A_{(s^+,s^-)}^{D,\sgn}(0,p)$
    according to \eqref{initialCondition}.
    \item Assume that we already have all values of $A_{(s^+,s^-)}^{D,\sgn}(t,p)$ for $D = 0,\cdots,D_{\max}$
    all possible choices of $(s^+,s^-)$ and $p\in\mathcal{P}_D$
    at specific time $t$.
    We evolve the system to obtain corresponding values of at time $t+\dt$ by the following steps.
    \begin{itemize}
        \item Evolve the system according to \eqref{eq_advection} for half time step $\dt/2$ by upwind scheme.
        If points on hypotenuse (the sum of all components are $T$) are involved,
            boundary condition \eqref{eq_boundaryCondition} is applied.
        \item Evolve the system according to \eqref{eq_source} for full time step $\dt$.
        If points on $(D_{\max}+1)$-dimensional simplex is involved,
        the method to close the system in \Cref{ClosureOfTheSystem}
         is applied.
        \item Evolve the system according to \eqref{eq_advection} for another half time step $\dt/2$ by upwind scheme.
        \item Compute the density matrix and observable at time $t+\dt$ according to \eqref{densityMatrixContinuous}
        and $O = \tilde{\rho}_{(+1,+1)}-\tilde{\rho}_{(-1,-1)}$.
    \end{itemize}
    \item Repeat the previous step to evolve the system iteratively.
\end{itemize}
Note that the evolution according to \eqref{eq_advection}\eqref{eq_source}
 can be written as matrix-vector multiplications.

==> sections/subsections/continuousLimitOfAs.tex <==
In this section, we would now like to explore the relation between the function $A(t,h)$ and the quantities $A_{k-\dk+1}(S_k, \cdots, S_{k-\dk+1})$. By the idea of the i-QuAPI method, the quantity $A_{k-\dk+1}(S_k, \cdots, S_{k-\dk+1})$ denotes the ensemble of all the discrete paths whose last segments of length $T$ are given by $S_{k-\dk+1}, \cdots, S_k$. This can be observed by applying 
\eqref{propagation} recursively, resulting in
\begin{equation}
  \begin{split}
	A_{k-\dk+1} (S_k,\cdots,S_{k-\dk+1})
	= &\sum_{S_{k-\dk},\cdots,S_0 \in\mathcal{S}^2} \Bigg[
	\mel{s_k^+}{\e^{-\ii H_0 \dt}}{s_{k-1}^+}
	\cdots
	\mel{s_1^+}{\e^{-\ii H_0 \dt}}{s_0^+}
	\mel{s_0^+}{\tilde{\rho}_s(0)}{s_0^-}\\
	& \mel{s_0^-}{\e^{\ii H_0\dt}}{s_1^-}
	\cdots
	\mel{s_{k-1}^-}{\e^{\ii H_0\dt}}{s_k^-} \\
	&\prod_{j_1=0}^k \prod_{j_2 = \max\{0, k - \dk\}}^{j_1}
	\exp \left( - (s_{j_1}^+ - s_{j_1}^-)
	 (\eta_{j_1,j_2} s_{j_2}^+ - \eta_{j_1,j_2}^* s_{j_2}^-) \right) \Bigg],
  \end{split} 
  \label{ExpressionA}
\end{equation}
where the summation symbol takes into account all the possible paths before the segment specified in the arguments.
In particular, when $k=\dk-1$,
 $A_0$ has the following expression:
\begin{equation}
  \begin{split}
	A_{0} (S_{\dk-1},\cdots,S_0) = &
	\mel{s_{\dk-1}^+}{\e^{-\ii H_0 \dt}}{s_{\dk-2}^+}
	\cdots
	\mel{s_1^+}{\e^{-\ii H_0 \dt}}{s_0^+}
	\mel{s_0^+}{\tilde{\rho}_s(0)}{s_0^-}\\
	& \mel{s_0^-}{\e^{\ii H_0\dt}}{s_1^-}
	\cdots
	\mel{s_{\dk-2}^-}{\e^{\ii H_0\dt}}{s_{\dk-1}^-} \\
	&\prod_{j_1=0}^{\dk-1} \prod_{j_2 = 0}^{j_1}
	\exp \left( - (s_{j_1}^+ - s_{j_1}^-)
	 (\eta_{j_1,j_2} s_{j_2}^+ - \eta_{j_1,j_2}^* s_{j_2}^-) \right).
	\label{ExpressionAInitial}
  \end{split}
\end{equation}
In what follows, our goal is to take the limit $\Delta t \rightarrow 0$ for $A_0$, and then extend the result to general values of $k$.

% We first deal with the bath part, which corresponds to the double product in \eqref{AinitialDefinition}. The result is given in the following lemma:
% \begin{lemma}
% 	\label{exponentialTermTriangle}
% 	The following limit holds. \zc{Shall we define $h$ on $(t,t+T]$ to make this lemma easier to write?}
% 	\begin{equation}
% 	    \begin{split}
% 		&\lim_{\dt\rightarrow 0}
% 		\prod_{j_1=0}^k \prod_{j_2 = \max\{0, k - \dk\}}^{j_1}
% 		\exp \left( - (s_{j_1}^+ - s_{j_1}^-)
% 		(\eta_{j_1-j_2} s_{j_2}^+ - \eta_{j_1-j_2}^* s_{j_2}^-) \right) \\
% 		=& \exp\left(-\int_{0}^{t+T} \dif \tau_1 \int_{\max\{0,\tau_1-T\}}^{\tau_1}\dif \tau_2
% 		\left(s^+(\tau_1)-s^-(\tau_1)\right)\left(s^+(\tau_2)\tilde{\eta}(\tau_1-\tau_2)
% 		-s^-(\tau_2)\tilde{\eta}^*(\tau_1-\tau_2)\right)
% 		\right)
% 		\end{split}
% 	\end{equation}
% 	where $t = (k-\dk)\dt$, $T = \dk\dt$ 
% 	and $s=\{s^+,s^-\}:[0,t+T]\rightarrow\mathcal{S}^2$
% 	represents the states of the system,
% 	being similar to $h$ in (\ref{hDefinitionAbstract}) 
% 	although the corresponding time intervals are different. For function $s$ here, the corresponding time interval
% 	is $[0,t+T]$, 
% 	representing the states of the system
% 	from the beginning of evolution
% 	to the current time ($t+T$).
% 	The whole interval is divided into two parts:
% 	\begin{itemize}
% 	    \item Time interval $[0,t)$:
% 	    in this interval, all possible choices of the states will be summed up as expressed in \eqref{ExpressionA}.
% 	    \item Time interval $[t,t+T]$:
% 	    in this interval, the states are given by the parameter $h$ of the variable $A$, which means
% 	    \begin{equation}
% 	        s(\tau+T) = h(\tau), 0\le\tau\le T.
% 	    \end{equation}
% 	\end{itemize}
	
% %	\begin{proof}
% %	    The proof is based on the definition of integral.
% %	    For a integrable function $f$ and $k\dt = t+T$,
% %	    $\dk\dt = T$.
% %	    \begin{equation}
% %	        \int_{0}^{t+T} \dif \tau_1 \int_{\max\{0,\tau_1-T\}}^{\tau_1} \dif \tau_2
% %	        f(\tau_1,\tau_2)
% %	        = \lim_{\dt\rightarrow 0}
% %	        \sum_{j_1=0}^{k} \sum_{j_2=\max\{0,k-\dk\}}^{j_1}
% %	        f(j_1\dt,j_2\dt)\dt^2.
% %	    \end{equation}
% %	    Replace $f$ by the integrand
% %	    $\left(s^+(\tau_1)-s^-(\tau_1)\right)\left(s^+(\tau_2)\tilde{\eta}(\tau_1-\tau_2)
% %		-s^-(\tau_2)\tilde{\eta}^*(\tau_1-\tau_2)\right)$,
% %		and the apply \Cref{continuoustau}.
% %		The limit holds as a result of 
% %		$\e^{a}\e^{b} = \e^{a+b}$ for any $a,b$.
% %	\end{proof}
% \end{lemma}
% This lemma is the direct result of the definition of Riemann integrals, and the conclusion has the form similar to \Cref{thm_propagator}. Here we omit the details of its proof.

We first take the limit of the system part, represented by the product of several bra-kets in \eqref{ExpressionAInitial}. Since the path segment $h$ is denoted by specifying the locations of spin flips, we choose to deal with the continuous segments of $h$ and the discontinuities in $h$ separately, requiring the following two lemmas:
\begin{lemma}
	\label{nonJumpPart}
	Suppose in the time interval $[\mathcal{T}_1,\mathcal{T}_2] = [k_1\dt,k_2\dt]$,
	 the state of the system remains unchanged, \textit{i.e.}
	 \begin{displaymath}
	 S_{k_1} = \cdots = S_{k_2} = S := (r^+,r^-).
	 \end{displaymath}
	 For fixed $\mathcal{T}_1$ and $\mathcal{T}_2$, it holds that
	\begin{gather*}
		\lim_{\dt\rightarrow 0} 
		\mel{s_{k_2}^+}{\e^{-\ii H_0\dt}}{s_{k_2-1}^+} \cdots
		\mel{s_{k_1+1}^+}{\e^{-\ii H_0\dt}}{s_{k_1}^+}
		= \e^{-\ii 
		\expval{H_0}{r^+} (\mathcal{T}_2-\mathcal{T}_1)}, \\
		\lim_{\dt\rightarrow 0} 
		\mel{s_{k_1}^-}{\e^{\ii H_0\dt}}{s_{k_1+1}^-} \cdots
		\mel{s_{k_2-1}^-}{\e^{\ii H_0\dt}}{s_{k_2}^-}
		= \e^{\ii \expval{H_0}{r^-} (\mathcal{T}_2-\mathcal{T}_1)}.
		\label{tempLable1}
	\end{gather*}
	\begin{proof}
		By the limit 
		$\e = \lim_{x\rightarrow 0}\left(1+x\right)^{1/x}$
		and Taylor expansion of the operator 
		$\e^{-\ii H_0\dt} = \id - \ii H_0 \dt + \mathcal{O}(\dt^2)$,
		\begin{equation*}
		\begin{split}
			&\lim_{\dt\rightarrow 0}
			 \mel{s_{k_2}^+}{\e^{-\ii H_0\dt}}{s_{k_2-1}^+} \cdots
		    \mel{s_{k_1+1}^+}{\e^{-\ii H_0\dt}}{s_{k_1}^+} \\
			=& \lim_{\dt\rightarrow 0}
			\expval{\id-\ii H_0 \dt + \mathcal{O}(\dt^2)}{r^+}
			^{(\mathcal{T}_2-\mathcal{T}_1)/\dt} \\
			=& \lim_{\dt\rightarrow 0}
			\left( 1- \ii\dt \expval{H_0}{r^+} + \mathcal{O}(\dt^2) \right)
			^{(\mathcal{T}_2-\mathcal{T}_1)/\dt} \\
			=&\e^{-\ii \expval{H_0}{r^+}
			 (\mathcal{T}_2-\mathcal{T}_1)}.
		\end{split}
		\end{equation*}
		The proof for the second limit is similar.
	\end{proof}
\end{lemma}
\begin{lemma}
	\label{JumpTheorem}
	When $s_k^+ \not= s_{k+1}^+$, the following limit holds.
	\begin{equation}
		\lim_{\dt\rightarrow 0}
		\frac{\mel{s_{k+1}^+}{\e^{-\ii H_0\dt}}{s_k^+}}{\dt}
		= -\ii \mel{s_{k+1}^+}{H_0}{s_k^+}.
	\end{equation}
	Similarly, when $s_k^- \not= s_k^-$, we have
	\begin{equation}
		\lim_{\dt\rightarrow 0}
		\frac{\mel{s_k^-}{\e^{\ii H_0 \dt}}{s_{k+1}^-}}{\dt}
		= \ii \mel{s_k^-}{H_0}{s_{k+1}^-}.
		\label{tempLabel2}
	\end{equation}
	\begin{proof}
		By Taylor expansion of $\e^{-\ii H_0\dt}$,
		\begin{align*}
			\lim_{\dt\rightarrow 0}
			\frac{\mel{s_{k+1}^+}{\e^{-\ii H_0 \dt}}{s_k^+}}{\dt}
			&=\lim_{\dt\rightarrow 0}
			\frac{\mel{s_{k+1}^+}{\id-\ii H_0 \dt + \mathcal{O}(\dt^2)}{s_k^+}}
			{\dt} \\
			&=\lim_{\dt\rightarrow 0}
			\frac{-\ii\dt\mel{s_{k+1}^+}{H_0}{s_k^+}+\mathcal{O}(\dt^2)}{\dt}
			= -\ii \mel{s_{k+1}^+}{H_0}{s_k^+}.
		\end{align*}
		The proof for (\ref{tempLabel2}) is similar.
	\end{proof}
\end{lemma}

This lemma shows that the quantity $A_0(S_{\dk-1}, \cdots, S_0)$ has magnitude $\dt^{-(p^+ + p^-)}$ if $s_k^{\pm}$ changes values $p^{\pm}$ times. Thus, it is natural to let the function $A(0,h)$ demonstrated in \Cref{RepresentationOfPaths} be the limit of $\dt^{p^+ + p^-} A_0(S_{\dk-1}, \cdots, S_0)$. We write down the result of such a limit in the following definition and theorem:

\begin{definition}
	\label{AinitialDefinition}
	For a function $h$ with the form
	\begin{equation}
		h^+ (t) = \sum_{j = 0}^{p^+} r_j^+ \mathbbm{1}_{[t_{j}^+,t_{j+1}^+)},
		\quad
		h^- (t) = \sum_{j = 0}^{p^-} r_j^- \mathbbm{1}_{[t_{j}^-, t_{j+1}^-)}
		\label{hFunction}
	\end{equation}
	where
    \begin{equation*}
        \begin{split}
            &r_{j}^+ \not= r_{j+1}^+ \text{ for } j=0,\cdots,p^+-1,
            \quad 
            r_j^- \not= r_{j+1}^-\text{ for } j=0,\cdots,p^--1 ;\\
            &0=t_0^+\leqslant t_1^+\leqslant\cdots \leqslant t_{p^+}^+ \leqslant t_{p^+ + 1}^+ = T,
            \quad
            0=t_0^-\leqslant t_1^-\leqslant\cdots \leqslant t_{p^-}^- \leqslant t_{p^- + 1}^- = T ;\\
            &\mathbbm{1}_{[a,b)}(x) = \begin{cases}
			1, \text{ if } x\in [a,b)\\
			0, \text{ if } x\notin [a,b)
		\end{cases}.
        \end{split}
    \end{equation*}
	the initial value $A(0,h)$ is defined to be
	\begin{equation}
	  \begin{split}
		A(0,h) = & \langle h^+(0) \vert \tilde{\rho}_s(0) \vert h^-(0)\rangle \\
		&\exp\left(-\int_{0}^{T} \dif \tau_1 \int_{0}^{\tau_1}\dif \tau_2
		(h^+(\tau_1)-h^-(\tau_1))(h^+(\tau_2)\tilde{\eta}(\tau_1-\tau_2)
		-h^-(\tau_2)\tilde{\eta}^*(\tau_1-\tau_2))\right) \\
		&\prod_{j^+=0}^{p^+ -1} \left(
		\e^{-\ii 
		\expval{H_0}{r_{j^+}^+}
		\left(t_{j^+ + 1}^+ - t_{j^+}^+\right)}
		(-\ii)
		\mel{r_{j^++1}^+}{H_0}{r_{j^+}^+}
		\right)
		\e^{-\ii \mel{r_{p^+}^+}{H_0}{r_{p^+}^+}
		\left(T - t_{p^+}^+\right)} \\
		&\prod_{j^-=0}^{p^--1} \left(
		\e^{\ii \expval{H_0}{r_{j^-}^-}
		\left(t_{j^-+1}^- - t_{j^-}^-\right)}
		(+\ii)\mel{r_{j^-}^-}{H_0}{r_{j^-+1}^-}
		\right)
		\e^{\ii\expval{H_0}{r_{p^-}^-}
		\left(T - t_{p^-}^-\right)}.
	  \end{split}
	  \label{initialCondition}
	\end{equation}
\end{definition}
With the definition above,
 the following theorem holds.
\begin{theorem}
	\label{AinitialLimit}
	The continuous and discrete versions of $A$ have the following relation:
	\begin{equation*}
		\lim_{\dt\rightarrow 0}
		\frac{A_{0} (S_{\dk-1},\cdots,S_0)}{\dt^{p^++p^-}}
		= A(0,h)
	\end{equation*}
	where $h$ represents the states of the system
	as discussed in \Cref{RepresentationOfPaths}
	and $(S_{\dk-1},\cdots,S_0)$ is given by
	$h$ according to the correspondence in \eqref{hS}.
	\begin{proof}
	    According to the definition of Riemann integral
	    and \eqref{eta_teta}
	    \begin{equation*}
	    \begin{split}
	        &\int_{0}^{T} \dif \tau_1 \int_{0}^{\tau_1}\dif \tau_2
		    (h^+(\tau_1)-h^-(\tau_1))(h^+(\tau_2)\tilde{\eta}(\tau_1-\tau_2)
		    -h^-(\tau_2)\tilde{\eta}^*(\tau_1-\tau_2))\\
		    = &\lim_{\dt\rightarrow 0}
		    \sum_{j_1 = 0}^{\dk-1} \sum_{j_2=0}^{j_1}
		    (s_{j_1}^+ - s_{j_1}^-)
		    \left(s_{j_2}^+ \tilde{\eta}(j_1\dt-j_2\dt)
		    -s_{j_2}^- \tilde{\eta}^*(j_1\dt-j_2\dt)\right) \dt^2 \\
		    = & \lim_{\dt\rightarrow 0} \sum_{j_1 = 0}^{\dk-1} \sum_{j_2=0}^{j_1}
		    (s_{j_1}^+ - s_{j_1}^-)
		    \left(s_{j_2}^+ {\eta}_{j_1,j_2}
		    -s_{j_2}^- {\eta}_{j_1,j_2}^*\right).
	    \end{split}
	    \end{equation*}
	    As for the system part,
	     \Cref{nonJumpPart} and \cref{JumpTheorem}
	     give the result,
	    noted that for each spin flip (discontinuity),
	     the order of $A_0(S_{\dk-1},\cdots,S_0)$
	     is raised by $\dt$.
	    Combining all the results together yields
	     the conclusion of the theorem.
	\end{proof}
\end{theorem}
The relation $A_0(S_{\dk}, \cdots, S_0) \sim \mathcal{O}(\Delta t^{p^+ + p^-})$ also agrees with the fact that the sum of $A_0(S_{\dk}, \cdots, S_0)$ for all possible choices of $S_{\dk}, \cdots, S_0$ converges to a finite number as $\Delta t \rightarrow 0$. Based on \Cref{JumpTheorem}, we can also observe from \eqref{ExpressionA} that $A_{k-\dk+1}(S_k, \cdots, S_{k-\dk+1}) \sim \mathcal{O}(\Delta t^{p^+ + p^-})$, where $p^+/p^-$ is the number of spin flips on the positive/negative branch of the path segment. Hence, when $t = (k-\dk) \dt >0$, we define $A(t,h)$ as the following quantity:
\begin{definition}
	\label{definitionACont}
	For $t\geqslant 0$ and $h$ given by (\ref{hFunction}),
	 the value of $A(t,h)$ is defined by
	\begin{equation*}
		A(t,h) = \lim_{\dt\rightarrow 0} 
		\frac{A_{k-\dk}(S_{k-1},\cdots,S_{k-\dk})}{\dt^{p^++p^-}}
	\end{equation*}
	where $(k-\dk)\dt=t$ and $\dk\dt=T$ is fixed.
\end{definition}
When $t=0$, Definition \ref{definitionACont} is consistent with 
  \Cref{AinitialDefinition} as a direct result of \Cref{AinitialLimit}. From the perspective of path integrals, $A(0,h)$ takes into account only the contribution of a single path $h$ of length $T$. However, when $t > 0$, the quantity $A(t,h)$ includes the contribution of infinite paths of length $t + T$ whose last segment of length $T$ agrees with $h$. Here we omit its expression of this form due to its tediousness.
